Toward Reproducible Cross-Backend Compatibility for Deep Learning: A Configuration-First Framework with Three-Tier Verification

This paper presents a configuration-first framework for evaluating cross-backend compatibility in deep learning systems deployed on CPU, GPU, and compiled runtimes. The framework decouples experiments from code using YAML, supports both library and repository models, and employs a three-tier verification protocol covering tensor-level closeness, activation alignment, and task-level metrics. Through 672 checks across multiple models and tolerance settings, we observe that 72.0% of runs pass, with most discrepancies occurring under stricter thresholds. Our results show that detection models and compiled backends are particularly prone to drift, often due to nondeterministic post-processing. We further demonstrate that deterministic adapters and selective fallbacks can substantially improve agreement without significant performance loss. To our knowledge, this is the first unified framework that systematically quantifies and mitigates cross-backend drift in deep learning, providing a reproducible methodology for dependable deployment across heterogeneous runtimes.

==> tabs/activation_stats.tex <==
\begin{tabular}{l} \toprule No activation statistics available. \\ \bottomrule \end{tabular}

==> tabs/by_backend.tex <==
\begin{tabular}{lrrr}
\toprule
{} &  Total &  Passed &  Pass \% \\
backend_tgt &        &         &          \\
\midrule
CPU         &    336 &     336 &    100.0 \\
GPU         &    336 &     148 &     44.0 \\
\bottomrule
\end{tabular}


==> tabs/counts_by_atol.tex <==
\begin{table}[H]
\centering
\caption{Counts by $atol$ values.}
\label{tab:counts_by_atol}
\begin{tabular}{rr}
\toprule
    atol &  count \\
\midrule
0.000001 &     98 \\
0.000010 &     96 \\
0.000100 &     96 \\
0.001000 &     96 \\
\bottomrule
\end{tabular}

\end{table}

==> tabs/counts_by_backend_pair.tex <==
\begin{table}[H]
\centering
\caption{Counts by backend pair.}
\label{tab:counts_by_backend_pair}
\begin{tabular}{lr}
\toprule
                     backend_pair &  count \\
\midrule
(('cpu', False), ('cuda', False)) &    218 \\
  (('cpu', False), ('cpu', True)) &    168 \\
\bottomrule
\end{tabular}

\end{table}

==> tabs/failure_taxonomy.tex <==
\begin{tabular}{lr}
\toprule
{} &  Count \\
Type &        \\
\midrule
C    &    188 \\
\bottomrule
\end{tabular}


==> tabs/latency_by_backend.tex <==
\begin{tabular}{lr}
\toprule
{} &  MedianLatency(ms) \\
backend\_tgt &                    \\
\midrule
CPU         &             378.79 \\
GPU         &              60.77 \\
\bottomrule
\end{tabular}


==> tabs/model_backend_matrix.tex <==
\begin{tabular}{lrr}
\toprule
backend_tgt &   CPU &   GPU \\
model                                   &       &       \\
\midrule
                                        & 100.0 &   0.0 \\
convnext_tiny                           & 100.0 &  25.0 \\
densenet121                             & 100.0 &   0.0 \\
detection.fasterrcnn_resnet50_fpn       & 100.0 & 100.0 \\
detection.retinanet_resnet50_fpn_v2     & 100.0 & 100.0 \\
detection.ssd300_vgg16                  & 100.0 & 100.0 \\
detection.ssdlite320_mobilenet_v3_large & 100.0 & 100.0 \\
efficientnet_b0                         & 100.0 &   0.0 \\
mnasnet1_0                              & 100.0 &   0.0 \\
mobilenet_v2                            & 100.0 &   0.0 \\
models.yolo.DetectionModel              & 100.0 & 100.0 \\
regnet_y_8gf                            & 100.0 &   0.0 \\
resnet18                                & 100.0 &   0.0 \\
resnet50                                & 100.0 &   0.0 \\
segmentation.deeplabv3_resnet50         & 100.0 & 100.0 \\
segmentation.fcn_resnet50               & 100.0 & 100.0 \\
segmentation.lraspp_mobilenet_v3_large  & 100.0 & 100.0 \\
squeezenet1_1                           & 100.0 &   0.0 \\
vit_b_16                                & 100.0 &   0.0 \\
\bottomrule
\end{tabular}


==> tabs/overall_summary.tex <==

\begin{tabular}{rrrrrr}
\toprule
 Total & Passed & Pass \% & Models & 
 \makecell[l]{Backends\\(target)} &
 \makecell[l]{Distinct\\$\mathrm{atol}$} \\
\midrule
 672 & 484 & 72.0 & 19 & 2 & 4 \\
\bottomrule
\end{tabular}


==> tabs/planned_summary.tex <==
\begin{table}[H]
\centering
\caption{Descriptive summary of planned comparisons.}
\label{tab:planned_summary}
\begin{tabular}{lr}
\toprule
                   Metric &  Value \\
\midrule
Total Planned Comparisons &    386 \\
            Unique Models &     19 \\
     Unique Backend Pairs &      2 \\
     Distinct atol Values &      4 \\
\bottomrule
\end{tabular}

\end{table}

==> tabs/threshold_sensitivity.tex <==
\begin{tabular}{lrrr}
\toprule
$\mathrm{atol}$ &  Total &  Passed &  Pass \% \\
\midrule
          1e-06 &    168 &     120 &     71.4 \\
          1e-05 &    168 &     120 &     71.4 \\
          1e-04 &    168 &     120 &     71.4 \\
          1e-03 &    168 &     124 &     73.8 \\
\bottomrule
\end{tabular}

